Backdoor Attacks with Input-unique Triggers in NLP

Backdoor attack aims at inducing neural models to make incorrect predictions for poison data while keeping predictions on the clean dataset unchanged, which creates a considerable threat to current natural language processing (NLP) systems. Existing backdoor attacking systems face two severe issues:firstly, most backdoor triggers follow a uniform and usually input-independent pattern, e.g., insertion of specific trigger words, synonym replacement. This significantly hinders the stealthiness of the attacking model, leading the trained backdoor model being easily identified as malicious by model probes. Secondly, trigger-inserted poisoned sentences are usually disfluent, ungrammatical, or even change the semantic meaning from the original sentence, making them being easily filtered in the pre-processing stage. To resolve these two issues, in this paper, we propose an input-unique backdoor attack(NURA), where we generate backdoor triggers unique to inputs. IDBA generates context-related triggers by continuing writing the input with a language model like GPT2. The generated sentence is used as the backdoor trigger. This strategy not only creates input-unique backdoor triggers, but also preserves the semantics of the original input, simultaneously resolving the two issues above. Experimental results show that the IDBA attack is effective for attack and difficult to defend: it achieves high attack success rate across all the widely applied benchmarks, while is immune to existing defending methods. In addition, it is able to generate fluent, grammatical, and diverse backdoor inputs, which can hardly be recognized through human inspection.

==> table/AttackResult.tex <==
\begin{table*}[htbp]
\setlength{\abovedisplayskip}{3pt} %%% 3pt 个人觉得稍妥，可自行设置

\setlength{\belowdisplayskip}{3pt} 
  \centering
  \small
    \begin{tabular}{ccccccccc}   
    \toprule
    Dataset & \multicolumn{2}{c}{AG's News} & \multicolumn{2}{c}{OLID} & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{Avg.} \\\cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}
    Attack Method & \multicolumn{1}{l}{ASR} & \multicolumn{1}{l}{CACC} & \multicolumn{1}{l}{ASR} & \multicolumn{1}{l}{CACC} & \multicolumn{1}{l}{ASR} & \multicolumn{1}{l}{CACC} & \multicolumn{1}{l}{ASR} & \multicolumn{1}{l}{CACC} \\\midrule
    RIPPLES & \textbf{89.39\%} & 89.06\% & \textbf{83.25\%} & 84.06\% & \textbf{90.16\%} & 89.01\% & \textbf{87.6\%} & \textbf{87.37\%} \\
    Syntactic & 78.42\% & \textbf{89.29\%} & 78.32\% & \textbf{84.3\%} & 78.25\% & 87.75\% & 78.33\% & 87.11\% \\
    LWS   & 85.97\% & 88.23\% & 74.87\% & 77.10\%  & 81.98\% & 84.51\% & 80.94\% & 83.28\% \\
    IADB   & 85.44\% & 86.28\% & 75.93\% & 81.92\% & 83.96\% & \textbf{90.49\%} & 80.57\% & 86.36\% \\\bottomrule
    \end{tabular}%
      \caption{Attack result on three datasets. }
  \label{tab:Experiment Result}
     \vspace{-5.0em}
\end{table*}

==> table/DefenseResult.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table*}[htbp]
%   \centering
%   \tiny
%     \begin{tabular}{cccccccccccccccccccccccc}
%     \toprule
%     Defense Method & \multicolumn{1}{c}{Dataset} & \multicolumn{2}{c}{RIPPLE} & \multicolumn{2}{c}{Syntactic} & \multicolumn{2}{c}{LWS} & \multicolumn{2}{c}{DBA} \\\midrule
%           &       & ASR   & CACC  & ASR   & CACC  & ASR   & \multicolumn{1}{c}{CACC} & ASR   & \multicolumn{1}{c}{CACC} \\\midrule
%      & AG's News & 10.62(78.77$\downarrow$)  & \underline{\textbf{88.61(0.45$\downarrow$)}}  & 69.83(8.53$\downarrow$)  & 84.01(6.92$\downarrow$)  & 75.97(10.00$\downarrow$)  & 87.74(0.49$\downarrow$)  & \underline{\textbf{82.24(3.20$\downarrow$)}} & 84.64(1.64$\downarrow$)  \\
%     ONION      & OLID  & 49.75(33.50$\downarrow$)  & \textbf{83.93(0.13$\downarrow$)} & \textbf{69.79(6.92$\downarrow$)} & 77.38(3.25$\downarrow$)  & 63.96(10.91$\downarrow$)  & \underline{77.07(0.03$\downarrow$)}  & \underline{67.32(5.00$\downarrow$)}  & 81.81(0.51$\downarrow$)  \\
%           & SST-2   & 16.78(73.38$\downarrow$)  & 88.00(1.01$\downarrow$)  & \underline{75.00(3.25$\downarrow$)}  & 88.82(-1.07$\uparrow$)  & 78.09(3.89$\downarrow$)  & \underline{86.75(-2.24$\uparrow$)}  & \textbf{80.23 (3.73$\downarrow$)} & \textbf{88.82(1.67$\downarrow$)} \\
%           & Avg.   & 25.72(61.88$\downarrow$)  & \underline{\textbf{86.85(0.53$\downarrow$)}} & 71.54(6.79$\downarrow$)  & 83.40(3.71$\downarrow$)  & 72.67(8.27$\downarrow$)  & 83.85(-0.57$\uparrow$)  & \underline{\textbf{76.60 (3.98$\downarrow$)}} & 85.09(1.27$\downarrow$)  \\\midrule
   
%     & AG's News & 36.28(53.11$\downarrow$)  & \underline{\textbf{88.48(0.58$\downarrow$) }} & 18.05(60.37$\downarrow$)  & 88.67(0.62$\downarrow$)  & 66.80(19.17$\downarrow$)  & 87.97(0.26$\downarrow$)  & \underline{\textbf{73.34 (12.10$\downarrow$)}} & 85.30(0.98$\downarrow$)  \\
%     Back-Translation      & OLID  & 56.96(26.29$\downarrow$)  & 83.53(0.53$\downarrow$)  & \textbf{73.65 (4.67$\downarrow$)} & \textbf{84.06 (0.24$\downarrow$)} & 67.30(7.57$\downarrow$)  & \underline{79.88(-2.78$\uparrow$)}  & \underline{67.09(5.23$\downarrow$)}  & 79.76(2.56$\downarrow$)  \\
%           & SST-2   & 49.01 (41.15$\downarrow$) & \underline{\textbf{86.81(2.20$\downarrow$)}} & 52.14(25.11$\downarrow$)  & 85.43(2.32)  & \underline{\textbf{66.44(15.54$\downarrow$)} } & 81.12(3.39$\downarrow$)  & 65.62 (18.34$\downarrow$) & 86.60(3.89$\downarrow$)  \\
%           & Avg.  & 47.42(40.18$\downarrow$)  & \underline{\textbf{86.27 (1.10$\downarrow$)}} & 47.95(30.38$\downarrow$)  & 86.05(1.06$\downarrow$)  & 66.85(14.09$\downarrow$)  & 82.99(0.29$\downarrow$)  & \underline{\textbf{68.68 (11.89$\downarrow$)}} &83.89(2.48$\downarrow$)  \\\midrule
%           & AG's News & 32.81(56.58$\downarrow$)  & 54.39(34.67$\downarrow$)  & -     & -     & \underline{\textbf{56.06 (29.91$\downarrow$)}} & 58.25(29.98$\downarrow$)  & 47.64(37.80$\downarrow$)  & \underline{\textbf{68.84 (17.74$\downarrow$)}} \\
%           Syntactic & OLID  & 30.69(56.26$\downarrow$)  & \textbf{76.86(7.20$\downarrow$)}  & 25.35(52.97$\downarrow$)  & 76.66(7.64$\downarrow$)  & \underline{\textbf{51.13 (23.74$\downarrow$)}} & \underline{73.16(3.94$\downarrow$)}  & 27.59(44.73$\downarrow$)  & 73.72(8.50$\downarrow$)\\
%           & SST-2  &49.01(41.15$\downarrow$) & 80.00(9.01$\downarrow$)  & 32.41(45.48$\downarrow$)  & \underline{79.34(8.41$\downarrow$)}  &  \textbf{\underline{63.43(18.55$\downarrow$)}} & 71.55(12.96$\downarrow$)  & 29.76(54.20$\downarrow$)  & \textbf{80.83(9.66$\downarrow$)}  \\
%           & Avg.   & 37.50(50.10$\downarrow$)  & 70.42(16.96$\downarrow$)  & 28.88(49.45$\downarrow$)  & \textbf{\underline{78.00(9.11$\downarrow$)}}  & \textbf{56.87(24.07$\downarrow$) }& 67.65(15.63$\downarrow$)  & 35.00(45.58$\downarrow$)  & 74.46(11.90$\downarrow$)  \\\bottomrule
%     \end{tabular}%
%       \caption{Defense result on three attack methods. The \textbf{blodfaced number} means the best performance on the dataset and the \underline{underlined number} means having the smallest declines, which is shown in brackets.}
%   \label{tab:DefenseResult}%
% \end{table*}%
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table*}[htbp]
%   \centering
%   \tiny
%   \caption{Defense result on three attack methods. The \textbf{blodfaced number} means the best performance on the dataset, both for the \textbf{A}ttack \textbf{S}uccess \textbf{R}ate(ASR) and the \textbf{C}lean \textbf{A}ccuracy.}
%     \begin{tabular}{cccccccccccccc}
%     \toprule
%     \multirow{2}[2]{*}{} & \multicolumn{1}{c}{\multirow{2}[2]{*}{Attack Method}} & \multicolumn{4}{c}{ONION}     & \multicolumn{4}{c}{Back-Translation} & \multicolumn{3}{c}{Avg.} &  \\\cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14}
%           &       & ASR   &$\Delta ASR$ & \multicolumn{1}{c}{CACC} &$\Delta CACC$  & ASR   &    $\Delta ASR$   & \multicolumn{1}{c}{CACC} & $\Delta CACC$ & \multicolumn{1}{c}{ASR} & $\Delta ASR$  & \multicolumn{1}{c}{CACC} &$\Delta CACC$  \\
%     \midrule
%     \multirow{4}[2]{*}{Ag's News} & RIPPLE & 10.62  & 78.77  & \multicolumn{1}{c}{\textbf{88.61 }} & \textbf{0.45 } & 36.28  & \multicolumn{1}{c}{53.11 } & \multicolumn{1}{c}{88.48 } & 0.58  & 23.45  & 65.94  & \textbf{88.55 } & 0.52  \\
%   & Syntactic & 69.83  & 8.59  & \multicolumn{1}{c}{84.01 } & 5.28  & 18.05  & \multicolumn{1}{c}{60.37 } & \multicolumn{1}{c}{\textbf{88.67 }} & 0.62  & 43.94  & 34.48  & 86.34  & 2.95  \\
%   & LWS   & 75.97  & 10.00  & 87.74  & 0.49  & 66.80  & \multicolumn{1}{c}{19.17 } & 87.97  & \textbf{0.26 } & 71.39  & 14.59  & 87.86  & \textbf{0.38}  \\
%   & DBA   & \textbf{82.24 } & 3.20  & 84.64  & 1.64  & \textbf{73.34 } & \multicolumn{1}{c}{\textbf{12.10 }} & 85.30  & 0.98  & \textbf{77.79 } & \textbf{7.65 } & 84.97  & 1.31  \\
%     \midrule
%     \multirow{4}[2]{*}{OLID} & RIPPLE & 49.75  & 33.50  & \multicolumn{1}{c}{\textbf{83.93 }} & 0.13  & 56.96  & \multicolumn{1}{c}{26.29 } & \multicolumn{1}{c}{83.53 } & 0.53  & 53.36  & 29.90  & \textbf{83.73 } & 0.33  \\
%       & Syntactic & \textbf{69.79 } & 8.53  & \multicolumn{1}{c}{77.38 } & 6.92  & \textbf{73.65 } & \multicolumn{1}{c}{\textbf{4.67 }} & \multicolumn{1}{c}{\textbf{84.06 }} & 0.24  & \textbf{71.72 } & 6.60  & 80.72  & 3.58  \\
%       & LWS   & 63.96  & 10.91  & 77.07  & \textbf{0.03 } & 67.30  & \multicolumn{1}{c}{7.57 } & 79.88  & \textbf{-2.78 } & 65.63  & 9.24  & 78.48  & \textbf{-1.38 } \\
%       & DBA   & 67.32  & \textbf{5.00 } & 81.81  & 0.51  & 67.09  & \multicolumn{1}{c}{5.23 } & 79.76  & 2.56  & 67.21  & \textbf{5.11 } & 80.79  & 1.53  \\\midrule
%       \multirow{4}[2]{*}{SST-2} & RIPPLE & 16.78  & 73.38  & \multicolumn{1}{c}{88.00 } & 1.01  & 49.01  & 41.15  & \multicolumn{1}{c}{\textbf{86.81 }} & \textbf{2.20 } & 32.90  & 57.27  & 87.41  & 1.61  \\
%       & Syntactic & 75.00  & 3.25  & \multicolumn{1}{c}{88.82 } & -1.07  & 52.14  & \textbf{26.11 } & \multicolumn{1}{c}{85.43 } & 2.32  & 63.57  & 14.68  & 87.13  & 0.63  \\
%       & LWS   & 78.09  & 3.89  & 86.75  & \textbf{-2.24 } & \textbf{66.44 } & 15.54  & 81.12  & 3.39  & 72.27  & \textbf{9.72}  & d83.94  & \textbf{0.58 } \\
%       & DBA   & \textbf{80.23 } & 3.73  & \textbf{88.82 } & 1.67  & 65.62  & 18.34  & 86.60  & 3.89  & \textbf{72.93 } & 11.04  & \textbf{87.71}  & 2.78  \\\bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}%
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
  \centering
    \begin{tabular}{cccccccc}
    \toprule
    \multirow{2}[0]{*}{Dataset} & \multirow{2}[0]{*}{Attack Method} & \multicolumn{2}{c}{ONION} & \multicolumn{2}{c}{Back-Translation} & \multicolumn{2}{c}{Avg.} \\\cmidrule(r){3-4}\cmidrule(r){5-6}\cmidrule(r){7-8}
          &       & ASR   & CACC  & ASR   & CACC  & ASR   & CACC \\\midrule
    \multirow{4}[0]{*}{Ag's News} & RIPPLE & 10.62\% & \textbf{88.61\%} & 36.28\% & 88.48\% & 23.45\% & \textbf{88.54\%} \\
          & Syntactic & 69.83\% & 84.01\%& 18.05\% & \textbf{88.67\%} & 43.94\% & 86.34\% \\
          & LWS   & 75.97\% & 87.74\% & 66.8\%  & 87.97\% & 71.39\% & 87.86\% \\
          & IDBA    & \textbf{82.24\%} & 84.64\% & \textbf{73.34\%} & 85.3\%  & \textbf{77.79\%} & 84.97\% \\\midrule
    \multirow{4}[0]{*}{OLID} & RIPPLE & 49.75\% & \textbf{83.93\%} & 56.96\% & 83.53\% & 53.355\% & \textbf{83.73\%} \\
          & Syntactic & 69.79\% & 77.38\% & \textbf{73.65\%} & \textbf{84.06\%} & \textbf{71.72\%} & 80.72\% \\
          & LWS   & 63.96\% & 77.07\% & 67.3\%  & 79.88\% & 65.63\% & 78.475\% \\
          & IDBA   & \textbf{73.13}\% & 81.81\% & 68.23 \% & 81.39\% & 70.68 \% & 81.22\% \\\midrule
    \multirow{4}[0]{*}{SST-2} & RIPPLE & 16.78\% & 88.00\%    & 49.01\% & \textbf{86.81\%} & 32.895\% & 87.405\% \\
          & Syntactic & 75.00\%    & 88.82\% & 52.14\% & 85.43\% & 63.57\% & 87.125\% \\
          & LWS   & 78.09\% & 86.75\% & 66.44\% & 81.12\% & 72.27\% & 83.935\% \\
          & IDBA   & \textbf{80.23\%} & \textbf{88.82\%} & \textbf{66.52\%} & 86.6\%  & \textbf{73.375\%} & \textbf{87.71\%} \\\bottomrule
    \end{tabular}%
      \caption{Defend result of different attack methods. For Onion we use the threshold where the model's performance decrease no more than 1\% on the clean validation dataset.}
        \label{tab:DefenseResult}%
\vspace{-5.0em}
\end{table*}%

==> table/Specifity.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
\setlength{\belowcaptionskip}{-0.cm}
  \centering
    \begin{tabular}{cc}
    \toprule
    Dataset & \multicolumn{1}{l}{Cross Accuracy} \\
    \midrule
    AG's News & 24.62\% \\
    OLID  & 29.77\% \\
    SST-2 & 26.09\% \\\bottomrule
    
    \end{tabular}%
    \caption{The cross-trigger accuracy on three datasets.}
  \label{tab:CrossTrigger}%
\end{table}%

